Constraining Hot Dark Matter Sub-Species with Weak Lensing and the Cosmic Microwave Background Radiation

Although it is well known that the bulk of dark matter (DM) has to be cold, the existence of an additional sub-dominant, hot species remains a valid possibility. In this paper we investigate the potential of the cosmic shear power spectrum to constrain such a mixed (hot plus cold) DM scenario with two additional free parameters, the hot-to-total DM fraction ($f_{\rm hdm}$) and the thermal mass of the hot component ($m_{\rm hdm}$). Running a Bayesian inference analysis for both the Kilo-Degree Survey cosmic shear data (KiDS) as well as the Cosmic Microwave Background (CMB) temperature and polarisation data from Planck, we derive new constraints for the mixed DM scenario. We find a 95 per cent confidence limit of $f_{\rm hdm}<0.08$ for a very hot species of $m_{\rm hdm}\leq20$ eV. This constraint is weakened to $f_{\rm hdm}<0.25$ for $m_{\rm hdm}\leq80$ eV. Scenarios with masses above $m_{\rm hdm}\sim200$ eV remain unconstrained by the data. Next to providing limits, we investigate the potential of mixed DM to address the clustering (or $S_8$) tension between lensing and the CMB. We find a reduction of the 2D ($\Omega_m - S_8$) tension from 2.9$\sigma$ to 1.6$\sigma$ when going from a pure cold DM to a mixed DM scenario. When computing the 1D gaussian tension on $S_8$ the improvement is milder, from 2.4$\sigma$ to 2.0$\sigma$.

==> cache_methods.tex <==
\underline{Linear power spectrum}: (add a part on wdm in CLass)\\
The linear power spectrum is computed using CLASS (Cite). It is run twice in every step, once for the forward modelling using only $\Lambda$CDM parameters and once with the mixed dark matter parameters to calculate $\sigma_8$ for the correct theory.  This is due to the fact that the Parimbelli emulator calculates a mixed dark matter correction to the non-linear power spectrum. 
The non-linear power spectrum is obtained using the revised halofit fitting function \cite{takahashi_revising_2012}. \\
\underline{Intrinsic alignment}:
Intrinsic alignment is the coherent alignment of galaxies with local structure due to tidal forces. As it impacts the orientation of galaxy shapes it is an important systematic effect to take into account in the modelling. For a review of different modelling approaches see \cite{krause_impact_2016} or \cite{jagvaral_intrinsic_2022} for an astrophysical subtle distinction. 
Here we used the strategy of \cite{hildebrandt_kids-450_2017}, with the decomposition as in (1) from \cite{heymans_kids-1000_2021}:
\begin{equation}\label{eq4}
C^{(ij)}_{\epsilon,\epsilon}(\ell)=C^{(ij)}_{G,G}(\ell)+C^{(ij)}_{GI}(\ell)+C^{(ij)}_{I,G}(\ell)+C^{(ij)}_{II}(\ell)
\end{equation}
The ij subscript denote the corellation between two redshift bins.The G and I stand respectively for "Galaxy" and "Intrinsic". The GG term is the one carrying the cosmological information, as it represents the correlation due to distortion by the matter field. The weight of the GI,IG and II terms are modelled using:
\begin{equation}\label{eq4}
F(z)=-A_{IA}C_1 \rho_{crit} \frac{\Omega_m}{D_+(z)}\left(\frac{1+z}{1+z_0}\right)^\eta\left(\frac{\bar{L}}{L_0}\right)^{\beta}
\end{equation}
Here we use $A_IA$ as the free parameter and fix $\eta=0$ and $\Beta=0$ in accordance with \cite{hildebrandt_kids-450_2017}. We fit $A_{IA}$ using:
\begin{equation}\label{eq4}
C_{I,G}(\ell),C_{G,I}(\ell) \propto F(z)  \ ; \ C_{G,G}(\ell) \propto   F(z)^2
\end{equation}

\underline{Baryonic feedback model}:

To account for baryon-driven feedback processes in the cosmic shear measurement we use the baryonic effect emulator from \cite{giri_emulation_2021}. This emulator uses physically motivated parameters to reproduce the matter power spectrum suppression from baryonic feedback proceses at $k>0.1Mpc/h$. The model is based on the adoption of a dark-matter baryon ($dmb$) profile of the halo: 
\begin{equation}\label{eq4}
\rho_{dmb}(r)=\rho_{clm}(r)+\rho_{gas}(r)+\rho_{cga}(r)
\end{equation}
The collision-less matter profile ($clm$) is composed of dark matter, stars of satellite galaxies and the stellar halo. The central galaxy profile ($cga$) represents the stars in the galaxies. The gas profile is fitted using five parameters: {$M_c,\mu,\Theta_{ej},\gamma,\delta$}. Two additional parameters {$\eta,\eta_\delta$} quantify the stellar to halo fraction, firstly $\eta$ for the stellar fraction in the satellite galaxies and halo stars and $\eta_d$ for the central galxy stars.\\
In \cite{giri_emulation_2021} it is shown that 3 parameters {$log^{10}M_c,\eta_\delta,\Theta_{ej}$} are sufficient to recover the power-spectrum suppression from the hydrodynamical simulations to a good accuracy, a prescription we follow to incorporate baryonic feedback into our analysis.
\\
\underline{Mixed Dark Matter Emulator}:

The parameters of the model are 

To evaluate the impact of mixed dark matter on the cosmic shear signal we use the data provided in Asgari et al. 
To model the Angular power spectrum we have:
\begin{equation}\label{eq4}
C_{E,l}=\frac{1}{2N_l}\int_{0}^{\infty} d\Mathcal{\ell}  \ \ell [W^l_{EE}(\ell)C_{EE}(\ell)+W^l_{EB}C_{BB}(\ell)] 
\end{equation}
with $N_l$ a normalization defined by 
\begin{equation}\label{eq4}
N_l =ln(\ell_{up,l})-ln(\ell_{lo,l})
\end{equation}
to ensure that the $\ell$ bin of the band power is logarithmically centred.
We extract the window functions $W^l_{EE}(\ell)$ from fig.1 in \cite{asgari_kids-1000_2021}. We have neglected the contributions of the B-modes in this analysis. 

\underline{Phase Space distribution} \\
Our warm/hot dark matter candidate is a sterile neutrino of the Dodelson Widrow type, with a phase space distribution normalized to fit the fractional energy density. As stated in Acero 2010 the phase space distribution is of the Fermi-Dirac type:
\begin{equation}\label{eq1}
f_0(q)=\frac{\chi}{\exp^{q-\chi}+1}
\end{equation}

By rescaling $f(p)$ we allow for the relation between $\omega_s$ and $f(p)$: 
\begin{equation}\label{eq1}
\omega_s=\Omega_s h_0^2=\frac{m}{\pi^2}\int dp  p^2 f(p) \frac{h^2}{\rho_c^o}
\end{equation}

As explained in Acero 2010, different models sharing {$\omega_s,\Delta N_{eff},<v_s>$} can have the same phenomenological effects, with $<v_s>$ the average velocity of the particle today.

